RankBooster: Visual Analysis of Ranking Predictions

Ranking is a natural and ubiquitous way to facilitate decision-making in various applications. However, different rankings are often used for the same set of entities, with each ranking method placing emphasis on different factors. These factors can also be multi-dimensional in nature, compounding the problem. This complexity can make it challenging for an entity which is being ranked to understand what they can do to improve their rankings, and to analyze the effect of changes in various factors to their overall rank. In this paper, we present RankBooster, a novel visual analytics system to help users conveniently investigate ranking predictions. We take university rankings as an example and focus on helping universities to better explore their rankings, where they can compare themselves to their rivals in key areas as well as overall. Novel visualizations are proposed to enable efficient analysis of rankings, including a Scenario Analysis View to show a high-level summary of different ranking scenarios, a Relationship View to visualize the influence of each attribute on different indicators and a Rival View to compare the ranking of a university and those of its rivals. A case study demonstrates the usefulness and effectiveness of RankBooster in facilitating the visual analysis of ranking predictions and helping users better understand their current situation.

==> EGauthorGuidelines-body.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.03, Dec 14, 2018


\title[RankBooster: Visual Analysis of Ranking Predictions]%
      {RankBooster: Visual Analysis of Ranking Predictions}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[Abishek Puri et al.]
{\parbox{\textwidth}{\centering
Abishek Puri$^{1}$\orcid{0000-0001-8945-6984},
Bon Kyung Ku$^{1}$\orcid{0000-0002-4534-8110},
Yong Wang$^{1}$\orcid{0000-0003-0177-1731},
Huamin Qu$^{1}$\orcid{0000-0002-3344-9694}
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering 
          $^1$ Hong Kong University of Science and Technology, Hong Kong
%        $^2$ Another Department to illustrate the use in papers from authors
%             with different affiliations
       }
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract}
   Ranking is a natural and ubiquitous way to facilitate decision-making in various applications. However, different rankings are often used for the same set of entities, with each ranking method placing emphasis on different factors. These factors can also be multi-dimensional in nature, compounding the problem. This complexity can make it challenging for an entity which is being ranked to understand what they can do to improve their rankings, and to analyze the effect of changes in various factors to their overall rank. 
In this paper, we present RankBooster, a novel visual analytics system to help users conveniently investigate ranking predictions. We take university rankings as an example and focus on helping universities to better explore their rankings, where they can compare themselves to their rivals in key areas as well as overall. Novel visualizations are proposed to enable efficient analysis of rankings, including a \textit{Scenario Analysis View} to show a high-level summary of different ranking scenarios, a \textit{Relationship View} to visualize the influence of each attribute on different indicators and a \textit{Rival View} to compare the ranking of a university and those of its rivals. A case study demonstrates the usefulness and effectiveness of RankBooster in facilitating the visual analysis of ranking predictions and helping users better understand their current situation.

%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see https://www.acm.org/publications/computing-classification-system/1998)
% \begin{classification} % according to https://www.acm.org/publications/computing-classification-system/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010352.10010381</concept_id>
<concept_desc>Computing methodologies~Collision detection</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010588.10010559</concept_id>
<concept_desc>Hardware~Sensors and actuators</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010584.10010587</concept_id>
<concept_desc>Hardware~PCB design and layout</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Visual analytics}
\ccsdesc[500]{Human-centered computing~Information visualization}


\printccsdesc   
\end{abstract}  
\begin{figure*}
  \includegraphics[width=\textwidth,height=7cm]{pictures/Teaser.png}
   \caption{The user interface showing multiple rival universities, where Scenario 13 is selected for further analysis. (A) the Scenario Analysis View, (B) the Relationship View where 4 scenarios have been selected for comparison, (C) the Rival Heat Map View, (D) the Rival Radar Chart View, (E) the Scenario List View. }
   	\label{fig:teaser}
\end{figure*}
\section{Introduction}

Ranking is a natural and ubiquitous way to help people make decisions in various applications, for example, finding a good restaurant and hotel for a trip, choosing the best university, and buying a suitable car. Many studies have been conducted to help people easily interpret rankings and make better decisions through visualization. Few studies, however, have focused on helping the entities (or items) being ranked, which we call ``rankees''.

Due to the wide usage of ranking companies, the impact of a low ranking can be substantial. For example, universities with a lower ranking receive less applications and private funding \cite{Rankings_Impact}. In this paper, we aim to tackle the following question \textit{how can we use visualization techniques to help universities efficiently interpret their rankings and analyze the effect of their actions on their ranking?} 

There are three reasons why this is a challenging question: multiple ranking systems and large number of entities, prediction uncertainties, and users' unfamiliarity with ranking prediction and visualization.

First, the sheer number of systems and methodologies for creating rankings creates complexity. Second, predictions are innately uncertain, and so the system must show the user the uncertainty. Third, many of the university administrators are not familiar with predictive analytics and visualization, requiring the system to be simple yet comprehensive.

Our research problem can be regarded as a Multi-Criteria-Decision-Making (MCDM) problem with the added complexity of uncertainty visualization. There have been many prior studies in the field of MCDM over the past decade \cite{weightlifter,mcdm_fisheries,mcdm_mograms,mcdm_top,krause2016interacting}, but they have generally focused on either high-level analysis of the tasks required to be solved \cite{high_level_MCDM} or aiding decision-making without any uncertainty involved in the variables {\cite{weightlifter}}. To the best of our knowledge, in the domain of ranking visualization, there has been no work attempting to aid rankees in their decision-making issue.

In this paper, we propose a visual analytics system, RankBooster, built in collaboration with university ranking experts. During this collaboration, we were able to create a set of tasks that could be generalized to other sets of entities who need to understand how to improve their ranking position in their ranking systems.

Our visual analytics system was used by our university to analyze their ranking position prior to their data submission. Our case study with the domain experts also shows the effectiveness of our approach.

Our major contributions can be summarized as follows:
\begin{itemize}
    \item A visual analytics system, RankBooster.
    \item A novel glyph visualization to show the relationship between the Indicators and the Attributes in ranking systems. 
    \item A case study with the domain experts highlighting the usability of the system.
\end{itemize}

%------------------------------------------------------------------------
\section{Related Work} 

As our work comes from the ranking visualization domain, we will list out key work in ranking visualization.

Part of the literature consists of works that aim to allow users to interact with the ranking system by modifying the weights or inputting their preferences. Works in this area include LineUp \cite{lineup}, Podium \cite{Podium}, and Rankit \cite{rankit}. However, they do not attempt to visualize any predictions of established rankings, focusing on existing rankings and making them more interactive and accessible. Other work has focused on looking at rankings over time, allowing users to observe trends and patterns. An example work in this area is RankExplorer \cite{rankexplorer}. While such works allow rankees to evaluate historical trends visually, they do not provide a way to evaluate scenarios in the future, or evaluate the effect of decisions made now. With regards to university rankings, which is the domain we will focus on in the paper, we could find only one other work \cite{dcpairs_uses_universities_ranking} that uses university rankings, but again their focus is on helping students make the decision, not the universities. Therefore, we claim that our perspective on this domain is a novel one.
% \subsection{MCDM Visualization}
% Work such as WeightLifter \cite{weightlifter}, TOP-Slider \cite{mcdm_top}, and moGrams \cite{mcdm_mograms} all provide ways of visualizing the solution space of an MCDM problem for different users. However, they all assume that, while the weight space can be uncertain, the function mapping the inputs and weights to the output is known. This means that there is no visualization that shows the uncertainty related to that mapping, which is a major part of the contribution. Another key difference is that, because our work is ranking-centric, our system visualizes the intermediate steps naturally, i.e. the Indicators, whereas WeightLifter focuses on the singular end goal. This is because WeightLifter was not specifically designed for the ranking domain. These are two key differences between our work and WeightLifter. The role of uncertainty in MCDM is well known, with a large body of work focusing on this issue in MCDM research \cite{mcdm_needs_uncertainty,issues_in_mcdm}[10], and it forms a major component of our problem as well. There has been work in the area of visualizing uncertainty in the mapping of the input space to the output space. Berger et. al \cite{mcdm_uncertainty_space} proposed a visual system that visualizes the uncertainty of the aforementioned mapping using parallel coordinates. However, their proposed system does not scale with the number of input and output variables. This can cause issues when there are a large number of variables that need to be visualized, which is the case in our research. A recent work by Krause et al. \cite{krause2016interacting} also explores how to visualize the results of a model in an agnostic way, which allows it to be used to solve MCDM problems. However, this work uses single views for every possible pair, resulting in a large cognitive overload when comparing many scenarios or many universities. The work also doesn't implicitly have a visualization for intermediate variables like Indicators, which is a feature our visual system must have. However the work provides a strong foundation upon which to base our system, as they do tackle uncertainty as well as the visualization of the relationship between attributes.  Other works have focused on domain-specific applications, such as the bio-medical domain \cite{mcdm_medical}, the environmental domain \cite{mcdm_uncertainty_flood_control}, and the fisheries domain \cite{mcdm_fisheries}. The proposed systems in these works apply to those specific domains and are not effectively transferable to the ranking domain. Therefore, in the domain of rankings, to the best of our knowledge no work has been done with respect to the uncertainty-aware version of the MCDM problem faced by rankees.

% \subsection{Uncertainty Visualization}
% A major challenge that is faced in this area is one that is ubiquitous in predictive modelling: uncertainty. Being able to visualize uncertainty in a meaningful way is a highly complex problem, and one that has spawned its own field within visualization. The important role of uncertainty is made clear by Sacha et. al \cite{uncertainty_guidelines_1}, providing us with an even stronger foundation for adding uncertainty analysis to our work. There are multiple surveys on uncertainty, in general or domain-specific cases, that have been conducted in the last few years \cite{uncertainty_survey_1,uncertainty_survey_2,uncertainty_survey_3}, providing a reference for those who want to know more.  In general, we found that the most relevant work to our paper came from two areas: visualizing uncertainty in a general pipeline, and domain-specific visualization of uncertainty.
% With regards to uncertainty in a general pipeline, the use of  visualization structures such as Box Plots \cite{boxplots}, Scatter Plots \cite{scatterplots}, and Glyphs \cite{glyphs} provide ways to convert uncertainty values into these forms and then insert them into a pipeline. Such structures as proposed in the paper were considered as alternative designs, which will be discussed in Section 6 in more detail. The work by Wu et al.  \cite{uncertainty_flow}, in terms of proposing new methods of quantifying and visualizing uncertainty, focused on improving the visualization of uncertainty during general analysis whilst Chen et al. \cite{QU_uncertainty} proposed new ways of quantifying uncertainty as well as a novel visualization, called an ``ensemble bar". Our work uses this novel visualization as a base upon which to create our own uncertainty visualization. The reader can refer to their work to find out more about the ensemble bar. We also took inspiration from the other works listed above when designing our system.




%-------------------------------------------------------------------------

\section{Background}
 
\subsection{Terminology}
 In this subsection, we explain key terminology used in the paper, through an example of a ranking system submission and result.
 
 First, raw data is collected on the rankees. These are the \textit{Attributes}. Then, the data is split into different groups and normalized across all rankees. These normalized groups are the \textit{Indicators}, and the normalized value for a given rankee in an Indicator is their \textit{Indicator Score}. Finally, all of a rankees Indicator Scores are inputted into a function which then gives them their \textit{Final Score}. These final scores are the basis of a rankees final rank.
 
 The question that is of interest to the rankee is \textit{What will be the Final Score given the values of the Attributes I am submitting?} To frame the question, we create a \textit{Scenario}, which consists of a set of Attributes and their values, the predicted Indicator Scores, and the predicted Final Score. Our system allows the user to evaluate scenarios individually or collectively.
 
 \subsection{Predictive Model Requirements}
 
 Our system assumes the user already has a model that can generate predictions of the Indicator Scores, along with some measure of uncertainty. It also assumes that the user already has a model that can generate predictions for other universities, along with some measure of uncertainty. 
 
 During our collaboration, an ensemble model which produced 100 predictions for each Indicator Score was used, with the range of the predictions providing us with the measure of uncertainty. 
 
 \subsection{Example Of A Scenario}
 
 As an example, we imagine a ranking system with 3 Attributes, coalesced into 2 Indicators, eventually creating a final score. In a given scenario, we have known values for the 3 Attributes. Then, we have predictions for the 2 Indicator Scores, as well as a prediction of the Final Score. These predictions are normalized to be between 1 and a 100 inclusive. For each prediction, we also have a measure of uncertainty. In our case, the uncertainty is the range of the 100 values produced by the model for each prediction. 

% In the ranking system pipeline (Fig. \ref{fig:info_pipeline}), the raw data of the university (Attributes) is used as a primary source of data in the system. Attributes can be classified into two types: Submitted Data (data which could be controlled, such as number of students) and Extraneous Variables (data which could not be controlled, such as academic reputation).

% Attributes are then used to calculate intermediate scores (Indicators). The precise method of conversion from Attributes to Indicators is unknown to the rankees. Each Indicator has a value normalized to a range, typically 1 to 100. The final score is then calculated using a known mapping from Indicator to Final Score. This score is used to rank the universities.

\subsection{Dataset Access}
Our dataset includes 5 years of data on over 400 universities. While the Indicator and Final Score are publicly available through the respective ranking systems websites, the Attribute values are not publicly available, requiring us to get the dataset from our collaborators.

%-------------------------------------------------------------------------
% \section{Data Processing}

% In this section we elucidate how we process the raw dataset into scenarios and generate uncertainty bounds for our predictions. We first present the Indicator prediction problem and our proposed solution. We then present the ranking position problem and our proposed solution. We further introduce the concept of ``Attribute influence on an Indicator" and how we calculate it.  Finally, we go through the structure of a scenario. 

% \subsection{Indicator Prediction Problem}
% The problem is to discover the mapping between the Attributes and the Indicators in the first layer. Below is a precise formulation of the problem:\\\\
% Let $I^y = \{I^y_1,I^y_2....I^y_N\}$ be the set of all Indicator values for a given year $y$.\\
% Let $A^y = \{A^y_1,A^y_2....A^y_N\}$ be the set of all Attribute values for a given year $y$.\\

% It is known there exists a function $G^{y+1}_i$ which maps Attribute values and unknown extraneous variables to a value for Indicator $i$ in the year $y+1$. This is either the function that would be used by the ranking systems in the case of a deterministic Indicator, or a function that, given enough extraneous data, would give an approximation approaching the truth for a subjective Indicator. Writing this more formally:

% $$G^{y+1}_i(A',Z) = I^{y+1}_i$$ Where $A'$ is any values assigned to the Attributes in set $A^y$ , $Z$ is a subset of all information, and $I^{y+1}_i$ is the value of the Indicator in the year $y+1$ given those assigned values occur. 

% However, this function is unknown, and so we must approximate it using a predictive model. This predictive model essentially gives us: $$^{*}G^{y+1}_i(A') = ^{*}I^{y+1}_i$$ where instead of getting the ``true" value we are getting a prediction. Notice that we remove $Z$ from this equation. This is because our predictive model has no access to those variables, and so can only use Attribute related data for its modelling.

% We first need to generate the optimal approximation functions for each Indicator. We used a Random Forest Regression (RF) Model for each of the Indicators, with the input being 3 years of historical data. This choice was made after testing other models such as a Recurrent Neural Network \cite{RNN}(RNN) (using 2 - 5 years of historical data) and k-NN, both of which returned less optimal results. 

% We then trained 100 RF models, each using different seed values and different partitions of the data-set for training and testing. These are used to generate 100 predictions per input array. The spread of these values give us an intuition about the uncertainty.

% A key point to note is that although we have mathematically modelled our solution as an approximate function, in reality we do not generate an analytic function. Rather, each model returns a prediction, and the collection of all predictions is used to create an approximation of the final value. Another key point is that the model structure described above is included in the paper so that the reader can understand what models the case studies are based on. In reality, our visual system is model-agnostic, as long as the model provides enough information to calculate uncertainty and influence as described in this section.
% \subsection{Ranking Position Problem}

% Once we have the overall score, calculated by summing the predictions for each indicator with the appropriate weightage, we then have to calculate a prediction for the ranking position next year. This is non-trivial, as we need to be able to account for other universities' movement as well. Therefore, we need a way to predict their Indicator values for the next year, even though we do not have the Attribute values for the current year for other universities. 

% To simplify the problem, we created three models of behavior for each university: Static, 1-Year, 2-Year. In the Static model, we assumed that the other universities stayed at the same position. In the 1-Year model, we assumed that the other universities grew at the same rate as in the last year. In the 2-Year model, we assumed that the other universities grew at the average growth rate of the last two years. These models were chosen by the experts, as they have used such behavioral approximations in their own work before. 

% Another simplification made was to only analyze the universities in the neighborhood, i.e. within 15 positions, of our university. For example, if the selected university was at Rank 20, we would only look at universities of Rank 5 to 35. This was because universities tend to move a limited number of positions, and we noticed that it is very rare for a university to move more than 20 positions.

% Using these two simplifications, we solve the problem by using the three models on all the universities in the neighborhood. For each university we choose the model that predicts the highest score, so as to make our recommendation conservative, and using this list of highest scores we calculate what our new position should be given our new score. If we are positioned at the top or at the bottom of the calculated neighborhood, we iteratively extend our window by five until that is no longer the case.

% It is once again important to note that these models were used in our work with HKUST OIR, but the visual system that we have developed would work on any models that were created to model rival universities' behavior. The models used for our work have been described for completeness.

% \subsection{Attribute Influence}

% When creating the predictions for the Indicators, an important piece of information is the influence of changes in the input on the prediction. This information is also important to visualize because it gives the user an idea as to the effect of changing the input variables without having to run a new simulation. We therefore visualize this influence in our system. 

% As mentioned in Section 4.1, our models are modelling a function that maps the Attribute values we input to a prediction of an Indicators value next year. Using this, we can define a quantitative value for the influence of this function to the input variables by using the partial derivative of the function with respect to a particular input variable. More formally: $$Inf^{I_i}_{A_j} = \frac{\partial ^{*}G^{y+1}_i(A')}{\partial A_j} |_{A'-A_j}$$ where $Inf^{I_i}_{A_j}$ is the Influence of Attribute j on Indicator i. 

% This method of sensitivity analysis is part of the OAT (One-At-a-Time) family of analytical tools \cite{saltelli2004sensitivity}. Methods of this family are useful in our case as we only need to evaluate the partial derivative at selected points, we do not need to get a general form. 

% We approximated the partial derivatives by using the finite difference method. Below is the formulation:

% $$Inf^{I_i}_{A_j} \approx \frac{^{*}G^{y+1}_i(A'-A_j,A_j=A_j+h) -^{*}G^{y+1}_i(A') }{h} $$ where h was empirically set at 0.001.  
% \subsection{Scenario Structure}
% Our main data structure for the visual system is the scenario. A scenario consists of four main parts: 

% \begin{itemize}
%     \item \textbf{The required changes for each Attribute}: Every Attribute that is to be submitted is given a value that this scenario has set it to. This value is given relative to the submitted value of the previous year, as the experts we talked to stated that the relative change is more important for them than the absolute change. 
%     \item \textbf{The generated predictions for each Indicator}: Every Indicator that has been selected for visualization is given an array of predicted values. In our case study we use 100 predicted values for each Indicator. 
%     \item \textbf{The influence of each Attribute on each Indicator}: For each Indicator we calculate the influence every Attribute has on that Indicator in this scenario. 
%     \item \textbf{The generated predictions for the final score and ranking}: There are 100 predicted values for the final score, created by sampling from the predictions of each Indicator. We then provide a matching change in ranking position for each of those aforementioned predicted values.
% \end{itemize}


% Throughout this paper, we will refer to the set of all Attributes, set of all Indicators, and set of all Final Values as components. We will refer to each individual member of the aforementioned components as a Variable.


%-------------------------------------------------------------------------
\section{Requirements Analysis}

Based on a survey of ranking experts, we were able to identify 3 main requirements of the system. 
\begin{itemize}
    \item \textbf{R1. Explore Scenarios Individually} 
    The system should be able to track a scenario from the submitted data to the final score. It should also show the relevant uncertainties, and identify Attributes and Indicators that will have the most impact on their rankings.
    
    \item \textbf{R2. Explore Scenarios As A Group}
    The system should be able to compare Attributes, Indicators, Final Scores, and uncertainties between scenarios. Users should also be able to filter and constrain the set of scenarios, and visualize a summary.
    
    \item \textbf{R3. Compare with Rival Universities} 
    The system should be able to directly compare a selected university with its rivals, focusing on predicted differences given a particular scenario.
\end{itemize}

% \subsection{Tasks for the System}

% From the aforementioned goals, we were able to create seven concrete tasks.
% \begin{itemize}
    
%     \item \textbf{T3. Compare Multiple Solutions}
%     The user should be able to compare the Attribute changes, predicted Indicator changes, and predicted final changes for multiple scenarios. Based on discussions with the experts, this task will involve at most four scenarios.
    
%     \item \textbf{T6. Compare multiple entities' solution sets}
%     The user should be able to look at multiple entities and their possible scenarios. This should be done in a way that allows the user to compare a particular scenario against the expected result of a rival entity, and also allows the user to compare a particular scenario against the set of possible scenarios of a rival entity.
%     \item \textbf{T7. Visualize a summary of the solutions}
%     The user should be able to view all the generated scenarios at a high-level, so as to have an overview of the entire set of scenarios as well as an easy way to select any individual solution for in-depth analysis. 
% \end{itemize}
    



%-------------------------------------------------------------------------
\section{Visual Design}
This section describes the usage of each view in our system, the design rationale for each view, and the interactions in each view.

\subsection{Scenario List View}
This view, shown in Fig.\ref{fig:teaser}(E), is a table, with each row of the table showing a summary of one scenario. This view partially satisfies \textbf{R2}, specifically providing a filterable and sort-able summary of all scenarios. It gives the user a simple interface by which to select particular scenarios for further analysis in the other views of the system. 

We show the change in the Attributes and the predicted change in Indicator Scores and Final Scores as bars. Here, the change is relative to the previous years values and scores respectively. The color represents whether the change is positive (green) or negative (red). 

% \subsubsection{Design Rationale}
% With regards to alternatives, we initially tried clustering the 2-D MDS projections of the scenarios. This would allow us to identify clusters of scenarios that are similar to each other. However, our users, found it confusing to interpret, as they thought the scenarios that were in the top left quadrant were better in some sense than those in other quadrants. This issue was resolved with a table design. 

% With regard to encoding the value of a scenario, we chose colored vertical bars because they were the most intuitive and space-minimizing out of the four bar designs that we came up with, namely colored horizontal bars, single colored horizontal bars, colored vertical bars, and single colored vertical bars. Single colored bars occupied too much space, as they used direction to denote positive or negative. When we showed the users horizontal bars, they complained that the visual made them dizzy. We therefore chose colored  bars.
% \subsubsection{Scalability and Generalization}
% With regards to scalability, we can view up to 40 scenarios with more scenarios accessible through the scrolling feature. This is sufficient for the users, who tended to be interested in the top 20 or 30 scenarios. The use of a table also makes the view generalizable.

\subsection{Scenario Analysis View}
This view, shown in Fig.\ref{fig:teaser}(A), consists of three columns of glyphs. The leftmost column has a glyph per Attribute, the middle column has a glyph per Indicator, and the rightmost column has a glyph each for the Final Score and the Final Rank. This view partially satisfies \textbf{R2}, showing a group summary of all the scenarios along with the uncertainty related to the predictions being made. It also partially satisfies \textbf{R3}, as multiple entities can be compared in this view.

Each glyph shows all the values for that object across all the selected scenarios, relative to the previous value of that object. For example, a glyph in the Attribute column would show all the values for a particular Attribute across all the scenarios, relative to the value of the Attribute in the previous year. This is encoded with a line chart, with the x-axis containing the relative values and the y-axis containing the frequency of appearance in the scenarios. 

We encode uncertainty by enhancing the ensemble bar from Chen et al. \cite{QU_uncertainty}. The enhancement consists of allowing multiple entities to be compared by superimposing each entities uncertainty on each other, whilst giving each entity a different color. The length of the bar along the glyph corresponds to the range of the uncertainty, with the lowest and highest relative values in the range of the prediction shown at the left and right of the bar respectively. In this encoding, negative values depict being below the previous years values. 

\subsection{Relationship View}
The view, shown in Fig.\ref{fig:teaser}(B), is a table of glyphs. Each row of the table represents a selected scenario, with each glyph in the row encoding information about the Attributes in the scenario and one Indicator in the scenario. Each column of the table represents one particular Indicator. This view partially satisfies \textbf{R1} and \textbf{R2}, specifically allowing the user to analyze the effects of the Attribute values of a scenario on the predicted Indicator Score and Final Score, whilst also allowing multiple scenarios to be compared with each other along the Indicator axis.

Any given glyph in this view is linked to a particular scenario and a particular Indicator. In Fig.\ref{fig:teaser}(B), the top-left glyph is linked to Scenario 0 and Indicator 1. The square shape of the glyph is due to the number of attributes; if there are more attributes, the shape would be a higher-sided polygon. The bar on the side of the glyph shows the value of a particular attribute in that scenario relative to the previous years value. The polygon is internally split equally amongst the attributes, with the shade signifying the relationship between that attribute and the indicator. The darker green the color of the section, the more the Indicator Score increases when the Attribute increases. The opposite is true if the color is a dark red. The curved bar on top of the glyph shows the predicted Indicator Score for that scenario with a line, and the maximum and minimum value of the Indicator Score is the total length of the bar. 

We determine the effect of an Attribute on the Indicator Score by perturbing the Attribute value and observing how that affects the models' Indicator Score prediction. The effect is normalized across all scenarios selected to be in the view.

% \subsubsection{Design Rationale}
% The critical piece of information to be encoded was the magnitude and direction of the influence of every relevant variable on the Indicator. We decided to also encode the value of the Indicator and the influencing variables for that particular scenario. This prevents the user from having to constantly switch between views to check that information. This follows the ``eyes beat memory" principle and reduces the visual workload of the user. 

% After finalizing the encoding scheme, we then clarified the key design requirements. It should not be cognitively demanding to compare the influence across Indicators as well as across multiple scenarios. This requirement guaranteed that the user would be able to effectively analyze the influence of an Attribute across Indicators in a particular scenario (Local Influence) and the influence of an Attribute for one Indicator across multiple scenarios (Global Influence), a key part of \textbf{(T4)}. To satisfy this requirement, our first design was a line chart for every Attribute-Indicator and Indicator-Final pair. This line chart would have the Attribute value on the x-axis and the Attribute influence on the Indicator on the y-axis. The design issue with this was that the users struggled to analyze Local Influence, as they had to look at a large number of graphs to get the information. Even though this design allowed for clear insight into the Global Influence, the trade off involving the loss of Local Influence analysis was significant, so this design was rejected. To allow for Local Influence analysis, we decided to use a scenario-based table layout, as this would guarantee that the user only had to look at a specific section to do the aforementioned analysis, instead of the entire view.

% Once we had the table layout, we had to decide how to represent each table cell. One alternative was to have a bar chart in each cell, where the height encoded the magnitude of the Attributes influence on the Indicator and the color of the bar encoded the direction. The vertical line next to each bar encodes the magnitude of the variables value in the scenario, and the color encodes the direction. We then use the horizontal bar below the bar chart to encode the value of the Indicator in the scenario, and the color encodes the direction. Whilst this design did capture all the information, the key issues were that it was a visually strenuous task to look at a column of such charts and compare the bars, making Global Influence analysis particularly challenging. Based on their feedback, we decided to create a new glpyh for the information.

% When designing the glyph, we wanted to encode the critical information with color, as Maguire et al. \cite{glyph_design_Maguire} found that color is the best way to encode such information. We had multiple glyph designs created and tested with the domain experts. This testing involved asking them questions that required Local Influence analysis and Global Influence analysis. The glyph that had the best overall performance was the one we eventually selected.
% \subsubsection{Scalability and Generalization}
% The design can support up-to 9 scenarios without there being a drop in the users ability to conduct Global Influence analysis. For our domain this was satisfactory; the users never required more than five in our case studies. In terms of its generalizability, it is possible that other domains would require more scenarios be compared to get a clear idea of the Global Influence. In those cases our design would not be applicable. However for domains where the number of scenarios viewed is controlled, our design can be used.
\subsection{Rival View}
This view has a heat map, shown in Fig.\ref{fig:teaser}(C), and a radar chart, shown in Fig.\ref{fig:teaser}(D). This view satisfies \textbf{R3}, allowing the user to compare predictions for different universities. The heat map encodes the probability that the users university will have a higher Indicator or Final Score than a rival university, given a particular scenario. Our users had 3 different methods for predicting the Indicator or Final Score for the rival universities; each method is given a row in the heat map. 

The radar chart encodes information about one method for predicting rival university Indicator and Final Scores, with the method selected via a drop-down list. Once a method is selected, the chart shows the predicted values, with the violin plot showing the uncertainty of that prediction as a distribution across all possible scores for that Indicator. This allows the user to  compare the rival universities expected value with the range of predictions made in the selected scenario. We can select a particular rival to have their values highlighted in the radar chart, for ease of use.

Having two views allows the user to go from a higher-level view of all methods across all rivals in the heat map, to a more focused view of one method in the radar chart. This abides by the "detail on demand" principle, as the user only goes to the radar char once they have noticed a method they want to focus on in the heat map.
% \subsubsection{Design Rationale}
%  The key piece of information to visualize was the probability of your university having a higher value than the rivals. As we had a probability mapping over two dimensions (Models on one axis, Indicators on another), we decided to use a heat map based on the analysis done by Bojko et al. \cite{bojko2009informative}. We also wanted another component in the view that would visualize the difference between the rivals and the selected university. As both the gap and the probability are critical pieces of information, we decided to use two components. For the second component, we initially thought of using a stacked bar chart or a radar chart. We asked the experts to try both to answer questions such as ``Which university is better than you overall?" and ``Is the gap in Indicator 1 large enough to compensate for the gap in the reverse direction in Indicator 4?". The experts preferred the radar chart as they said that having three or four colors in a bar chart got very confusing; the radar chart was easier to look at.
 
% \subsubsection{Scalability and Generalization}
% The heat map does scale with the number of models, but for a significantly large number of models, it would not suffice.  However, in such cases the focus of the analysis would have to be primarily rival based, which would mean they would require a system that was rival-analysis-centric. So for our use case, it is sufficiently scalable.

% \subsection{Interactions}

% We have six main interactions to facilitate the user experience of our system. These interactions tie the various views together to form one cohesive visual system.

% \begin{itemize}
%     \item \textbf{Left-Clicking a scenario:} This will generate the rival heat map and star view for that particular scenario. It will also create purple markers in the Scenario Analysis View and purple bar in the uncertainty range.
    
%     \item \textbf{Right-Clicking a scenario:} This will generate a row in the relationship view. 

%     \item \textbf{Left and Right Markers on the uncertainty bar:} This will filter all scenarios who have a simulation result outside the bar.

%     \item \textbf{Left and Right Markers on the line charts:} This will filter all scenarios who have changes for that variables outside the bar.

%     \item \textbf{Submitting an edited scenario:} This will update that particular scenario in the Scenario List View. It will also propagate the changes to all other affected views.

%     \item \textbf{Sorting By column title in the views:} This will sort a view by the column variable.

%     \item \textbf{Sorting By Attribute in the Relationship View:} This will sort the scenarios in the Relationship view by the selected Attribute, while enlarging the corresponding quadrant. Shown in Fig. \ref{fig:interactions}.
% \end{itemize}

% These interactions can be used in conjunction with each other, providing the user with even more interactivity.

\subsection{Implementation Details}
Our visual system was built using Vue.js, with a Python backend server. All the models were built using Python with scikit-learn.

%-------------------------------------------------------------------------
\section{Evaluation}

To evaluate our system, we conducted a case study and an interview with the experts to evaluate the overall effectiveness of the system.
\begin{figure}
 \centering
 \includegraphics[width=\linewidth]{pictures/today_shot.png}
 \caption{The main findings in the case study. (A) shows the variance in prediction for SFRI, and the two peaks in ISRI. It also shows the change in distribution after the filtering is applied. (B) shows the differences in the two selected scenarios for I4, I5, and I6. The highlighted quadrant corresponds to the first attribute. (C) shows the selected scenarios' uncertainty bound and position relative to other scenarios. (D) shows the distribution of predictions for the selected scenario, with the focus being on I1's shape.}
 \label{fig:case_studies}
 \end{figure}
\subsection{Finding Optimal Data Submission For a Ranking System}

 University A (``Uni") was in the process of submitting data to QS. They have a range of values that could be submitted for each attribute, and wanted to use the system to decide what to submit. The user was a female expert from Uni. 

She first selected Uni and inputted her submission range in the panel at the far left of Fig.\ref{fig:teaser}, which generated 1511 scenarios \textbf{(R2)}.

She noticed that the expected changes in Student Faculty Ratio Indicator (``SFRI") and International Student Ratio Indicator (``ISRI") had a lot of variation, while the other indicators didn't \textbf{(R2)}. She therefore decided to keep only those scenarios that have a predictive value larger than 0 for those two indicators, using the Scenario Analysis View.  She then noticed that there are two peaks of predicted values for ISRI, so she focused in on the second peak \textbf{(R2)}. The filtering had left 108 scenarios Fig.\ref{fig:case_studies}(A). She expressed surprise that there was such a large spread of values for SFRI and ISRI, stating this was an interesting insight. 

She now focused on the differences between the scenarios that remained after filtering. She decided to focus on the influence of the first attribute, as Uni had the most leeway on this attribute, so she sorted by this attribute and selected the first and last scenario to analyse more closely \textbf{(R2)} Fig.\ref{fig:case_studies}(B). She immediately noticed that the Local Influence was different in I4, I5, and I6.The change in the attribute had also caused the influence of other attributes to change, with some increasing and others decreasing Fig.\ref{fig:case_studies}(B). In particular, when the chosen attribute was the main influencer of I6 only when it had a negative change \textbf{(R1)}. She noted it down for further analysis with her team later. 

She now wanted to focus on the values for submission, so she selected the scenario matching one of the discrete values, to view it in the Scenario Analysis View in context of all scenarios \textbf{(R2)}Fig.\ref{fig:case_studies}(C). She immediately noticed that for SFRI, her selected scenario seemed to be predicting the average value, but the uncertainty was heavily biased in the negative direction \textbf{(R1)}. This bias in the negative direction implies that there is a significant possibility of the real outcome being below the predicted value, and so it could be risky to completely rely on the predicted value. She further investigated the scenario using the radar chart Fig.\ref{fig:case_studies}(D). Here she noticed that for I1, there is a bottom heavy distribution, so in her view that was enough evidence to discount this scenario with regards to I1. Similarly, the other values are viewed and, based on analysis in the same vein as above, she decided on a particular value set for data submission.
 
The case study shows how insights can be gained with regards to the optimality of the data points in the set of submittable values, as well as with regards to the relationship between the attributes and the indicators. 

% \subsection{Comparing Personal Performance To Rival Universities}

% In this case study, an expert from University A (``Uni") had pre-selected a particular scenario, and wanted to analyze this scenario in the context of its rival universities. He also wanted to look at the possible positions of the rival universities in the next year. 

% He first selected Uni for analysis and then added the rivals. For the constraints, he varied the values in his selected scenario by 5\%. The constraints on the simulations run from the perspective of the rivals was set to $\pm$3\% of their previous years data \textbf{(T5)}. 

% He first noticed that, with regards to the final score, Uni was expected to do poorly against its competitors, assuming they submitted the optimal values for their attributes to QS \textbf{(T6)}. This is shown in Fig.\ref{fig:case_studies}(E). This was an important insight for the expert. 

% He then selected his particular scenario to analyze in the rival view. The important thing to reiterate is that the models used in the rival view are the three mentioned in Section 4.2, allowing for comparisons between the predictions of these fixed model types to the predictions garnered from varying their previous years data by 3\%. The expert was surprised to find that in I1, I2, and I3, his university showed zero probability of defeating its rival universities, except for ``HKPolyU" \textbf{(T6)}. This is shown in Fig.\ref{fig:case_studies}(G) and was noted down as an important insight. As he looked at the row ``HKPolyU-Static", he surmised that the probability of surpassing HKPolyU was significant. He wanted to know what was the expected margin of defeat, so he looked at the star chart view and selected ``HKPolyU" on ``Static" mode. The result is shown in Fig.\ref{fig:case_studies}(F). He noticed that the gaps for I1, I2, I3 were not substantial \textbf{(T4)}, but the gaps for I4, I5, I6 were significantly large, predicting huge victory over the rival. This was noted down as a useful insight by the expert.

% This case study showed how the system could be used to compare a university to its rivals, either by generating scenarios for the rivals or by using fixed models of prediction. It also shows how those two methods listed above can also be compared to see the differences in the models' prediction.

% \subsection{Expert Interview}
% We kept in constant communication with the experts throughout the design process. This communication took the form of weekly meetings. Once the system was completed, we interviewed the experts. The feedback can be split into two distinct areas.

% \textbf{Visual System and Interactions}
% The experts felt that the system was highly intuitive; they appreciated having clearly segregated views providing varying amounts of detail, and the transition from a high level overview to a scenario specific or rival specific view was deemed to be smooth and easy to understand. One expert said that she could ``go from analyzing hundreds of scenarios to focusing on a handful without any issue" with the system. 

% \textbf{Gaining Insights}
% The practicality of the system with regards to the tasks that they have to complete was also praised. One expert mentioned that when they are not submitting rankings data they are still analyzing what would be the effect of various policy decisions on the ranking position, and the system allows them to conduct such analysis and provide nuanced analysis of policy effects. This comment highlighted that the system is not just for use during the data submission season. 

% Overall the experts had a highly favorable impression of the system and used it during the 2019 data submission for QS. 
\section{Discussion and Conclusion}

In this paper, we propose RankBooster, an interactive visual analytics system to help users conveniently investigate ranking predictions to understand the reasons of the ranking. We take university rankings as an example, working closely with the domain experts to generate requirements and build out the system. Our case study demonstrates how RankBooster can be be used to analyze scenarios and decide on the optimal data submission.

However, it is not without limitations. First, our analysis assumes that the attributes are independent of each other. Whilst this assumption is used in our domain, it may not always hold in other domains. Second, our evaluation is limited to universities specifically, further evaluation would need to be done with other domains to fully verify its usability in a more general setting. Tackling these issues will form the bulk of our future work in this area.


% This ne system was iteratively designed with constant communication with the domain experts, and each design choice was rigorously made. Our system was used during the data submission period in 2019 for the QS ranking system, highlighting the practical usage of our system. Our case studies as well as the positive feedback from our expert interview also highlight the usability of the system. 



% In this work, we formulate the problem faced by rankees, using the university ranking domain for our design study. This formulation results in the formation of a set of tasks faced by rankees when they are analyzing ranking data as well as submitting data to the ranking institutions. We then propose a visual system, RankBooster, which allows rankees to complete the collated tasks in an efficient manner. The system was iteratively designed with constant communication with the domain experts, and each design choice was rigorously made. Our system was used during the data submission period in 2019 for the QS ranking system, highlighting the practical usage of our system. Our case studies as well as the positive feedback from our expert interview also highlight the usability of the system. 








\iffalse

%-------------------------------------------------------------------------
% \section{Discussion}

% Our discussion with the experts as well as the case study we conducted show our systems high degree of usability. The fact that our system was used during the data submission period of this year is further proof of the practicality of the system. We discuss the received feedback below.

% There are 3 main limitations of our system, both when its used by the ranking domain experts and when it is extended to other domains.
% \begin{itemize}
%     \item  We do not analyze the dependence between Attributes or the dependence between Indicators, even though intuitively such dependence is possible. 
%     \item  Our underlying data does not have to be university rankings and the system should be able to adjust to other ranking systems. g rankees, creating a system that can be used by all ranking domains.
%     \item If you want to compare one scenario over multiple ranking systems, you must run the system once for each model and then manually compare. 
% \end{itemize}

% In general, our system is able to accomplish all the tasks set out after discussion with our university ranking domain experts. The major future work direction would be to look at augmenting the system with more intra-relationship analysis as well as making it more general so that any rankee from any domain can use the system efficiently.
% %-------------------------------------------------------------------------
% \section{Conclusion}

% In this work, we formulate the problem faced by rankees, using the university ranking domain for our design study. This formulation results in the formation of a set of tasks faced by rankees when they are analyzing ranking data as well as submitting data to the ranking institutions. We then propose a visual system, RankBooster, which allows rankees to complete the collated tasks in an efficient manner. The system was iteratively designed with constant communication with the domain experts, and each design choice was rigorously made. Our system was used during the data submission period in 2019 for the QS ranking system, highlighting the practical usage of our system. Our case studies as well as the positive feedback from our expert interview also highlight the usability of the system. 

% In future work we aim to generalize our approach to other domains, with the goal being to create a one-stop-shop for rankees looking to do such analysis on their data. We also aim to further analyze the intra-relationships of the variables, extending our analysis even further. 
\fi


%-------------------------------------------------------------------------

%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
% bibtex
\bibliographystyle{eg-alpha-doi}
\bibliography{egbibsample}

% biblatex with biber
% \printbibliography                

%-------------------------------------------------------------------------
\end{document}

